A semi-Lagrangian discontinuous Galerkin (DG) -- local DG method for solving convection-diffusion equations

In this paper, we propose an efficient high order semi-Lagrangian (SL) discontinuous Galerkin (DG) method for solving linear convection-diffusion equations. The method generalizes our previous work on developing the SLDG method for transport equations (J. Sci. Comput. 73: 514-542, 2017), making it capable of handling additional diffusion and source terms. Within the DG framework, the solution is evolved along the characteristics; while the diffusion term is discretized by the local DG (LDG) method and integrated along characteristics by implicit Runge-Kutta methods together with source terms. The proposed method is named the `SLDG-LDG' method and enjoys many attractive features of the DG and SL methods. These include the uniformly high order accuracy (e.g. third order) in space and in time, compact, mass conservative, and stability under large time stepping size. An $L^2$ stability analysis is provided when the method is coupled with the first order backward Euler discretization. Effectiveness of the method are demonstrated by a group of numerical tests in one and two dimensions.

==> Review/review.tex <==
\section{Review of SLDG and LDG methods}
\label{sec2}
\setcounter{equation}{0}
%\setcounter{figure}{0}
%\setcounter{table}{0}

\subsection{SLDG method formulated based on an adjoint problem}
\label{sec2.1}
First, we briefly review SLDG formulation for the following 1D linear transport problem
\beq\label{eq2:1}
\frac{\partial u}{\partial t} +\frac{\partial}{\partial x}(a(x,t)u) = 0 ,\quad  x \in [x_a,x_b],
\eeq
with  given initial condition and proper boundary conditions.  $a(x,t)$ is assumed to be continuous with respect to $x$ and $t$.  For more detailed algorithm, we refer the readers to \cite{cai2017high}.

The formulation starts with a partition of the computational domain $[x_a,x_b]$ into $N$ elements: 
\begin{align}
\label{eq2:2}
x_a = x_{\frac{1}{2}}<x_{\frac{3}{2}}<\cdots<x_{N+\frac{1}{2}} = x_b,
\end{align}
with $I_j = [\xL,\xR]$ denoting an element of length $\bigtriangleup x_{j}=\xR-\xL$ for $j=1,2,\cdots,N$.  $\Dt$ represents the time discretization step.
 
Both numerical solution and test function belong to the finite dimensional approximation space
%\begin{center}
%$V^k_h=\{v_h:v_h|_{I_j} \in P^k(I_j),j=1,2,\cdots,N \}$, 
%\end{center}
\beq
\label{eq2:3}
V^k_h=\{v_h:v_h|_{I_j} \in P^k(I_j),j=1,2,\cdots,N \}
\eeq
where $P^k(I_j)$ denotes the set of polynomials of degree at most $k$ over $I_j$ with $k \geq 0$.

Partition of domain and the discontinuous finite element space are defined the same way as $(\ref{eq2:2})$ and $(\ref{eq2:3})$ for the following problems.

In order to update the approximation numerical solution $u^{n+1}$ at the time level $t^{n+1}$ over $I_j$, we adopt the weak formulation of characteristic Galerkin method proposed in \cite{childs1990characteristic}, in which the time-dependent test function $\psi(x,t)$ satisfies the adjoint problem with $\forall \Psi(x,t^{n+1}) \in P^k(I_j)$,
\begin{equation}
\label{eq2:4}
\begin{cases}
\psi_t+a(x,t)\psi_x=0, \quad t \in [t^n,t^{n+1}],\\
\psi(x,t=t^{n+1})=\Psi(x,t^{n+1}),
\end{cases}
\end{equation}
with $t^n$ denoting the $n$-th time level.  From $(\ref{eq2:4})$, we can see that test function $\psi(x,t)$ stays constant along the trajectory $\frac{dx}{dt}=a(x,t)$.  It was also demonstrated in \cite{guo2014conservative} that
\beq
\label{eq2:5}
\frac{d}{dt}\int_{\widetilde{I}_j(t)} u(x,t) \psi(x,t) dx = 0,
\eeq
where $\widetilde{I}_j(t)$ is a dynamic interval bounded by characteristics emanating from cell boundaries of $I_j$ at $t=t^{n+1}$ (in Figure $\ref{schematic_1d(a)}$).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h!]
\centering
\subfigure[Dynamic interval $\widetilde{I}_j(t)$]{
\label{schematic_1d(a)}
\begin{tikzpicture}
\begin{scope}[thick]

\draw[black] (0+1,0) node[left] {} -- (6+1,0) node[right]{$t^{n}$};
\draw[black] (0+1,2) node[left] {$$} -- (6+1,2)  node[right]{$t^{n+1}$};

\draw[snake=ticks,segment length=2.4cm] (0.6+1,2) -- (3+1,2) node[above] {\scriptsize $\xL$};
\draw[snake=ticks,segment length=2.4cm] (3+1,2) -- (5.4+1,2) node[above] {\scriptsize$\xR$};

\draw[snake=ticks,segment length=2.4cm] (0.6+1,0) -- (3+1,0);
\draw[snake=ticks,segment length=2.4cm] (3+1,0) -- (5.4+1,0);
\draw[snake=ticks,segment length=2.4cm] (5.4+1,0) -- (6+1,0);

\fill [black] (3+1,2) circle (2pt) node[] {};
\fill [black] (5.4+1,2) circle (2pt) node[] {};

\draw[-latex,dashed](3+1,2)node[left,scale=1.3]{$$} 
      to[out=200,in=70] (3+1-1.4,0) node[above left=0pt] {\scriptsize $x_{\jL}^\star$}; 
 \fill [blue] (3+1 -1.4,0) circle (2pt) node[] {};

\draw[-latex,dashed](5.4+1,2)node[left,scale=1.3]{$$} 
      to[out=200,in=70] ( 5.4+1-1.4,0) node[above right=2pt] {\scriptsize $x_{\jR}^\star$};
\fill [blue] (5.4+1-1.4,0) circle (2pt) node[] {};

\draw[black] (3+1-1,1) node[left] {} -- (5.4+1-1,1) node[right]{}node[above left=0pt] {\scriptsize $\widetilde{I}_j(t)$}; 

\draw[snake=ticks,segment length=2.4cm] (0.6+1,0) -- (3+1,0) node[above ] {\scriptsize $I_j^{*}$};

\draw[snake=brace,mirror snake,red,thick] (3+1-1.4,0) -- (3+1,0) node[below left = 2.5pt] {$I^{*}_{j,1}$};

\draw[snake=brace,mirror snake,red,thick] (3+1,0) -- (5.4+1-1.4,0) node[below left = 2.5pt]{$I^{*}_{j,2}$};

\end{scope}
\end{tikzpicture}
}

\subfigure[Interpolation of $\psi(x,t^n)$]{
\label{schematic_1d(b)}
\begin{tikzpicture}
\begin{scope}[thick]

\draw[black] (0+1,0) node[left] {} -- (6+1,0) node[right]{$t^{n}$};
\draw[black] (0+1,2) node[left] {$$} -- (6+1,2)  node[right]{$t^{n+1}$};

\draw[snake=ticks,segment length=2.4cm] (0.6+1,2) -- (3+1,2) node[above] {\scriptsize $\xL$};
\draw[snake=ticks,segment length=2.4cm] (3+1,2) -- (5.4+1,2) node[above] {\scriptsize $\xR$};

\draw[snake=ticks,segment length=2.4cm] (0.6+1,0) -- (3+1,0);
\draw[snake=ticks,segment length=2.4cm] (3+1,0) -- (5.4+1,0);
\draw[snake=ticks,segment length=2.4cm] (5.4+1,0) -- (6+1,0);

\fill [black] (3+1,2) circle (2pt) node[] {};
\fill [black] (5.4+1,2) circle (2pt) node[] {};
\fill [black] (3+1+0.5,2) circle (2pt) node[] { };
\fill [black] (5.4+1-0.5,2) circle (2pt) node[] {};

\fill [blue] (3+1 -1.4,0) circle (2pt) node[] {};
\fill [blue] (5.4+1-1.4,0) circle (2pt) node[] {};
\fill [blue] (3+1+0.5-1.4,0) circle (2pt) node[] { };
\fill [blue] (5.4+1-0.5-1.4,0) circle (2pt) node[] {};

\draw[-latex,dashed](3+1,2)node[left,scale=1.3]{$$} 
      to[out=200,in=70] (1.6+1,0) node[above left=0pt] {\scriptsize $x_{\jL}^\star$}; 

\draw[-latex,dashed](5.4+1,2)node[left,scale=1.3]{$$} 
      to[out=200,in=70] ( 4+1,0) node[above right=2pt] {\scriptsize $x_{\jR}^\star$};
 
\draw[-latex,thick](3+1+0.5,3)node[right,scale=1.0]{\scriptsize $x_{j,p}$}
      to[out=260,in=100] (3+1+0.5,2) node[] {};

\draw[-latex,thick](3+1+0.5,2)node[right,scale=1.0]{} 
      to[out=200,in=70] (3+1+0.5-1.4,0) node[] {};

\draw[-latex,thick](3+1+1-1.4,-0.4)node[right=0pt,scale=1.0]{\scriptsize $(x_{j,p}^\star,\Psi(x_{j,p}) )$ $\rightarrow$ $\psi^\star(x)$ } node[below right=8pt,scale=0.8]{}                to[out=120,in=330] (3+1+0.5-1.4,0) node[] {};

\draw[-latex,thick](5.4+1-0.5,2)node[right,scale=1.0]{} 
      to[out=200,in=70] (5.4+1-0.5-1.4,0) node[] {};

\end{scope}
\end{tikzpicture}
}

\caption{Schematic illustration of the SLDG formulation in one dimension.  }
\label{schematic_1d}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

From $(\ref{eq2:5})$, the following equation holds:
\beq
\label{eq2:6}
\int_{I_j} u^{n+1} \Psi(x,t=t^{n+1}) dx = \int_{I_j^{*}} u^n \psi(x,t=t^n) dx,
\eeq
where $I_j^{*}=[\xl,\xr]$ is called upstream cell interval at time level $t^n$ and $I_j^{*}=\widetilde{I}_j(t=t^n)$.

For notation simplicity, $(\ref{eq2:6})$ is denoted as
\beq
\label{eq2:7}
\left(u^{n+1},\Psi(x,t^{n+1})\right)_{I_j} = \left(u^n,\psi(x,t^n)\right)_{I_j^{*}},
\eeq
where $(\cdot,\cdot)_{I_j}$ stands for the inner product on $I_j$.
%$\xl$ is located by solving final value problem
%\beq
%\begin{cases}
%\f{dx(t)}{dt}=a(x(t),t)\\
%x(t=t^{n+1})=\xL
%\end{cases}
%\eeq
%with high order numerical integrator such as fifth order Runge-Kutta method given in \cite{butcher2016numerical}.  $\xr$ can be achieved similarly.

 As can be seen in Figure $1(a)$, there may exist two overlaps $I^{*}_{j,1}$ and $I^{*}_{j,2}$.  In general, there can be many overlapping sub-intervals $I^{*}_{j,l}$ between $I^{*}_j$ and the background Eulerian intervals.  Correspondingly, the right hand side (RHS) of $(\ref{eq2:7})$ can be approximated by
\beq
\label{eq2:8}
\left(u^n,\psi(x,t^n)\right)_{I_j^{*}} \approx \displaystyle{\sum_l}\int_{I^{*}_{j,l}}u^n\psi^{*}(x,t=t^n)dx.
\eeq
Recall that $\psi(x,t)$ maintains its value along the trajectory according to $(\ref{eq2:4})$.  $\psi^{*}(x,t^n)$ can be reconstructed uniquely by interpolating $\psi(x,t^n)$ with points $(x^{*}_{j,p},\psi(x^{*}_{j,p}))=(x^{*}_{j,p},\Psi(x_{j,p}))$ (in Figure $\ref{schematic_1d(b)}$), where $x_{j,p}$ are the $k+1$ many interpolation points which be chosen as the Gauss-Lobatto points (the midpoint if $k=0$) over $I_j$ and $x^{*}_{j,p}$ are located by solving the final value problem
\beq
\label{eq2:9}
\begin{cases}
\f{dx(t)}{dt}=a(x(t),t)\\
x(t=t^{n+1})=x_{j,p}
\end{cases}
\eeq
at $t^n$ with high order numerical integrator such as fifth order Runge-Kutta method given in \cite{butcher2016numerical}.


\subsection{LDG for approximating second order derivatives}
\label{sec2.2}
For simplicity, we'll recall the semi-discrete LDG scheme for one dimensional second order spatial derivative
\beq
\label{eq2:10}
\epsilon u_{xx}, \quad x\in[x_a,x_b]
\eeq
with $\epsilon \geq 0$, given initial and boundary conditions.

$(\ref{eq2:10})$ can be rewritten as the following first order system
\beq
\label{eq2:11}
\begin{cases}
%u_t=p\\
%p=q_x\\
\epsilon u_{xx}=\epsilon q_x,\\
q=u_x.
\end{cases}
\eeq

%The time discretization can be realized by Runge-Kutta method with strong stability preserving property.  
For spatial discretization, find $u_h,q_h \in V^k_h$ such that, for all test functions $v_h,p_h\in V^k_h$, $ j =1,2,\cdots,N$,
%\begin{align}
%\inj (u_h)_{xx} v_h dx&=\epsilon \inj (q_h)_x v_h dx\\
%&=\epsilon \left[\widehat{q_h}_{\jR}(v_h)^{-}_{\jR}-\widehat{q_h}_{\jL}(v_h)^{+}_{\jL}-\inj q_h (v_h)_x dx\right],
%\end{align}
%
%\begin{align}
%\inj q_h p_h dx &= \inj (u_h)_x p_h dx\\
%&=\widehat{u_h}_{\jR}(p_h)^{-}_{\jR}-\widehat{u_h}_{\jL}(p_h)^{+}_{\jL}-\inj u_h (p_h)_x dx
%\end{align}
\begin{subequations}\label{eq2:12}
\begin{align}
\epsilon \inj (u_h)_{xx} v_h dx&=\epsilon \inj (q_h)_x v_h dx=\epsilon \left[\widehat{q_h}_{\jR}(v_h)^{-}_{\jR}-\widehat{q_h}_{\jL}(v_h)^{+}_{\jL}-\inj q_h (v_h)_x dx\right],\label{eq2:12a}\\
\inj q_h p_h dx &= \inj (u_h)_x p_h dx=\widehat{u_h}_{\jR}(p_h)^{-}_{\jR}-\widehat{u_h}_{\jL}(p_h)^{+}_{\jL}-\inj u_h (p_h)_x dx,\label{eq2:12b}
\end{align}
\end{subequations}
with $\widehat{\cdot}$ denoting the numerical fluxes at the cell interfaces.  The diffusion fluxes need to be chosen from alternating directions considering stability reason. In other words,
\begin{align}
\label{eq2:13}
\widehat{q_h} = (q_h)^{-}, \quad     \widehat{u_h} = (u_h)^{+};
\end{align}
or
\begin{align}
\label{eq2:14}
\widehat{q_h} = (q_h)^{+}, \quad    \widehat{u_h} = (u_h)^{-}.
\end{align}
Notice that $q_h$ is solved explicitly in terms of $u_h$ in $I_j$ from $(\ref{eq2:12b})$ and then $(u_h)_{xx}$ can be attained after plugging $q_h$ from $(\ref{eq2:12b})$ in $(\ref{eq2:12a})$.  In short, $(u_h)_{xx}$ on $I_j$ can be recovered only by using information from nearby intervals, namely $I_{j-1}$, $I_j$ and $I_{j+1}$.



